Elemental Abundance Ratios in Stars of the Outer Galactic Disk. IV. A New Sample of Open Clusters

We present radial velocities and chemical abundances for nine stars in the old, distant open clusters Be 18, Be 21, Be 22, Be 32, and PWM 4. For Be 18 and PWM 4, these are the first chemical abundance measurements. Combining our data with literature results produces a compilation of some 68 chemical abundance measurements in 49 unique clusters. For this combined sample, we study the chemical abundances of open clusters as a function of distance, age, and metallicity. We confirm that the metallicity gradient in the outer disk is flatter than the gradient in the vicinity of the solar neighborhood. We also confirm that the open clusters in the outer disk are metal-poor with enhancements in the ratios [alpha/Fe] and perhaps [Eu/Fe]. All elements show negligible or small trends between [X/Fe] and distance (< 0.02 dex/kpc), but for some elements, there is a hint that the local (RGC < 13 kpc) and distant (RGC > 13 kpc) samples may have different trends with distance. There is no evidence for significant abundance trends versus age (< 0.04 dex/Gyr). We measure the linear relation between [X/Fe] and metallicity, [Fe/H], and find that the scatter about the mean trend is comparable to the measurement uncertainties. Comparison with solar neighborhood field giants shows that the open clusters share similar abundance ratios [X/Fe] at a given metallicity. While the flattening of the metallicity gradient and enhanced [alpha/Fe] ratios in the outer disk suggest a different chemical enrichment history to the solar neighborhood, we echo the sentiments expressed by Friel et al. that definitive conclusions await homogeneous analyses of larger samples of stars in larger numbers of clusters. Arguably, our understanding of the evolution of the outer disk from open clusters is currently limited by systematic abundance differences between various studies.

==> tab06.tex <==
\begin{deluxetable}{lllrrrrrrrrrr}
\tabletypesize{\tiny}
\tablecolumns{9} 
\tablewidth{0pc} 
\tablecaption{Equivalent Widths for Program Stars \label{tab:ews}}
\tablehead{ 
\colhead{Wavelength (\AA)} &
\colhead{Species} & 
\colhead{LEP (eV)} &
\colhead{$\log gf$} &
\colhead{Be18 1163} &
\colhead{Be18 1383} &
\colhead{Be21 T50} &
\colhead{Be21 T51} &
\colhead{Be22 414} &
\colhead{Be22 643} &
\colhead{Be32 16} &
\colhead{Be32 18} &
\colhead{PWM RGB1} 
}
\startdata
 6300.30 &  8.0 &     0.00 &  $-$9.72 &  \ldots &    38.7 &  \ldots &    38.9 &    48.4 &   114.0 &    24.9 &    32.6 &    39.9 \\
 6363.78 &  8.0 &     0.02 & $-$10.19 &  \ldots &    20.8 &  \ldots &    20.3 &    27.3 &    83.2 &    16.3 &    11.9 &    31.0 \\
 5688.19 & 11.0 &     2.11 &  $-$0.42 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   120.7 &  \ldots &  \ldots \\
 6154.23 & 11.0 &     2.10 &  $-$1.53 &    60.8 &    75.0 &    74.6 &    73.2 &    77.8 &  \ldots &    44.3 &    50.6 &   111.8 \\
 6160.75 & 11.0 &     2.10 &  $-$1.23 &    83.8 &    97.6 &    97.9 &    96.0 &   103.6 &  \ldots &    68.1 &    71.1 &  \ldots \\
 5711.09 & 12.0 &     4.35 &  $-$1.83 &   122.5 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   105.5 &  \ldots &  \ldots \\
 6318.72 & 12.0 &     5.11 &  $-$1.97 &    63.0 &  \ldots &    67.0 &  \ldots &    66.5 &  \ldots &    53.2 &    46.9 &  \ldots \\
 6319.24 & 12.0 &     5.11 &  $-$2.22 &    43.9 &  \ldots &    41.1 &  \ldots &    40.6 &  \ldots &    37.4 &    37.0 &  \ldots \\
 6319.50 & 12.0 &     5.11 &  $-$2.43 &  \ldots &  \ldots &    31.5 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 6965.41 & 12.0 &     5.75 &  $-$1.51 &  \ldots &  \ldots &  \ldots &    47.0 &  \ldots &    42.7 &  \ldots &  \ldots &    50.5 \\
 7387.69 & 12.0 &     5.75 &  $-$0.87 &    73.7 &    66.6 &    75.3 &    71.9 &    65.0 &    63.9 &    63.3 &    68.6 &    82.0 \\
 6696.02 & 13.0 &     3.14 &  $-$1.34 &    60.1 &    73.9 &    71.8 &    71.8 &    81.6 &  \ldots &    51.4 &    57.4 &  \ldots \\
 6698.67 & 13.0 &     3.14 &  $-$1.64 &    45.6 &    52.2 &    46.2 &    57.8 &    54.7 &    94.0 &    27.6 &    31.1 &    86.5 \\
 5665.55 & 14.0 &     4.92 &  $-$1.92 &    51.8 &    58.0 &    63.3 &    62.2 &    58.0 &  \ldots &    48.1 &    54.2 &    67.5 \\
 5690.43 & 14.0 &     4.93 &  $-$1.72 &    42.2 &    54.0 &    62.1 &    57.5 &    57.8 &    55.8 &    49.8 &    56.6 &    56.4 \\
 5701.10 & 14.0 &     4.93 &  $-$1.93 &  \ldots &    40.4 &    48.9 &    45.9 &    43.0 &  \ldots &    44.8 &    50.5 &  \ldots \\
 5772.15 & 14.0 &     5.08 &  $-$1.75 &  \ldots &  \ldots &    65.9 &    61.3 &    60.2 &  \ldots &    53.5 &    61.5 &  \ldots \\
 5793.07 & 14.0 &     4.93 &  $-$1.77 &  \ldots &    52.8 &    55.7 &    49.8 &    52.8 &    65.6 &    48.4 &    55.0 &    47.4 \\
 5948.55 & 14.0 &     5.08 &  $-$1.07 &    82.6 &    86.4 &    90.6 &    88.6 &    81.4 &  \ldots &    78.4 &    89.0 &    95.1 \\
 6125.02 & 14.0 &     5.61 &  $-$1.48 &  \ldots &    40.4 &    41.1 &    39.7 &  \ldots &  \ldots &    37.2 &    34.9 &  \ldots \\
 6145.01 & 14.0 &     5.62 &  $-$1.38 &    35.4 &    29.6 &    36.8 &    36.2 &    35.9 &    27.7 &    35.6 &    38.2 &    32.3 \\
 6155.13 & 14.0 &     5.62 &  $-$0.70 &    73.3 &    72.1 &    80.1 &    76.2 &    78.5 &  \ldots &    71.0 &    79.1 &    77.3 \\
 6741.63 & 14.0 &     5.98 &  $-$1.75 &  \ldots &  \ldots &  \ldots &    20.8 &    16.3 &  \ldots &    13.4 &    15.0 &  \ldots \\
 6848.57 & 14.0 &     5.86 &  $-$1.61 &    19.2 &    12.3 &  \ldots &    17.5 &    15.5 &    21.3 &    21.7 &    25.7 &  \ldots \\
 7405.77 & 14.0 &     5.61 &  $-$0.63 &    94.1 &    89.4 &    95.0 &    96.0 &    88.1 &    70.8 &    93.1 &    95.5 &    80.4 \\
 7800.01 & 14.0 &     6.18 &  $-$0.70 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    46.9 &    51.9 &  \ldots \\
 4847.31 & 20.0 &     2.93 &  $-$1.40 &    71.1 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    97.9 \\
 5260.39 & 20.0 &     2.52 &  $-$1.72 &    53.4 &    64.3 &  \ldots &    62.4 &    70.0 &    95.1 &    42.2 &    45.9 &    93.1 \\
 5261.70 & 20.0 &     2.52 &  $-$0.58 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   100.2 &   114.2 &  \ldots \\
 5512.98 & 20.0 &     2.93 &  $-$0.45 &  \ldots &   112.9 &  \ldots &   110.3 &   116.5 &  \ldots &    92.8 &    96.8 &  \ldots \\
 5581.97 & 20.0 &     2.52 &  $-$0.56 &   119.4 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   100.5 &   109.2 &  \ldots \\
 5590.11 & 20.0 &     2.52 &  $-$0.57 &   115.4 &   124.7 &  \ldots &   123.5 &   124.2 &  \ldots &    95.5 &  \ldots &  \ldots \\
 5867.56 & 20.0 &     2.93 &  $-$1.57 &    35.7 &    54.3 &    48.9 &    48.0 &    51.1 &  \ldots &    32.9 &    32.4 &    97.5 \\
 6161.30 & 20.0 &     2.52 &  $-$1.27 &    97.7 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    87.8 &  \ldots \\
 6166.44 & 20.0 &     2.52 &  $-$1.14 &    99.2 &   117.1 &   105.9 &   108.9 &   115.3 &  \ldots &    80.3 &    89.5 &  \ldots \\
 6169.04 & 20.0 &     2.52 &  $-$0.80 &   118.2 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   109.4 &  \ldots \\
 6169.05 & 20.0 &     2.52 &  $-$0.80 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   109.4 &  \ldots \\
 6169.56 & 20.0 &     2.53 &  $-$0.48 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   115.0 &  \ldots &  \ldots \\
 6455.60 & 20.0 &     2.52 &  $-$1.29 &    99.4 &   111.1 &   101.9 &   101.8 &   103.5 &  \ldots &    73.0 &    75.1 &  \ldots \\
 6471.66 & 20.0 &     2.53 &  $-$0.69 &   117.1 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   100.3 &   112.1 &  \ldots \\
 6499.65 & 20.0 &     2.52 &  $-$0.82 &   119.3 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    99.5 &   104.9 &  \ldots \\
 4465.80 & 22.0 &     1.74 &  $-$0.11 &  \ldots &  \ldots &    72.8 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 4562.62 & 22.0 &     0.02 &  $-$2.60 &  \ldots &    95.0 &    76.9 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 4617.25 & 22.0 &     1.75 &     0.45 &    97.3 &   114.3 &   106.6 &   105.7 &  \ldots &  \ldots &    84.6 &    91.8 &  \ldots \\
 4656.47 & 22.0 &     0.00 &  $-$1.29 &   124.7 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 4758.12 & 22.0 &     2.25 &     0.48 &    73.2 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 4759.27 & 22.0 &     2.26 &     0.57 &  \ldots &  \ldots &    83.4 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 4820.41 & 22.0 &     1.50 &  $-$0.39 &   105.5 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    92.0 &  \ldots \\
 4840.87 & 22.0 &     0.90 &  $-$0.45 &   115.2 &  \ldots &   119.7 &  \ldots &  \ldots &  \ldots &   100.0 &   104.0 &  \ldots \\
 4913.62 & 22.0 &     1.87 &     0.22 &    93.6 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    83.6 &  \ldots \\
 4926.15 & 22.0 &     0.82 &  $-$2.11 &    46.9 &    73.8 &  \ldots &    62.7 &  \ldots &  \ldots &    33.2 &    31.0 &   111.4 \\
 5009.65 & 22.0 &     0.02 &  $-$2.20 &    99.3 &  \ldots &  \ldots &   109.9 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 5016.16 & 22.0 &     0.85 &  $-$0.52 &   121.7 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 5043.59 & 22.0 &     0.84 &  $-$1.68 &  \ldots &  \ldots &  \ldots &    78.4 &  \ldots &  \ldots &    53.0 &    57.6 &  \ldots \\
 5045.42 & 22.0 &     0.85 &  $-$1.94 &  \ldots &    89.1 &  \ldots &  \ldots &  \ldots &  \ldots &    46.6 &  \ldots &  \ldots \\
 5062.11 & 22.0 &     2.16 &  $-$0.41 &  \ldots &  \ldots &    69.1 &  \ldots &  \ldots &  \ldots &    34.7 &  \ldots &  \ldots \\
 5071.47 & 22.0 &     1.46 &  $-$1.01 &    76.5 &   105.9 &    93.2 &    87.9 &  \ldots &  \ldots &    54.4 &    61.4 &  \ldots \\
 5145.46 & 22.0 &     1.46 &  $-$0.52 &  \ldots &  \ldots &  \ldots &    95.9 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 5201.12 & 22.0 &     2.09 &  $-$0.69 &    63.7 &    65.7 &    64.9 &    52.1 &    81.3 &  \ldots &    34.2 &    29.9 &  \ldots \\
 5219.70 & 22.0 &     0.02 &  $-$2.24 &   101.4 &  \ldots &   110.9 &   118.3 &  \ldots &  \ldots &    72.3 &    80.2 &  \ldots \\
 5223.65 & 22.0 &     2.09 &  $-$0.50 &    49.6 &    66.0 &  \ldots &  \ldots &    73.7 &  \ldots &    40.2 &    43.8 &  \ldots \\
 5295.78 & 22.0 &     1.07 &  $-$1.58 &    55.2 &    82.0 &    68.2 &    70.3 &    84.7 &  \ldots &    43.1 &    44.6 &  \ldots \\
 5366.65 & 22.0 &     0.82 &  $-$2.53 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   118.7 \\
 5460.47 & 22.0 &     0.05 &  $-$2.75 &    77.9 &   112.1 &    85.6 &  \ldots &  \ldots &  \ldots &    49.8 &    52.3 &  \ldots \\
 5490.15 & 22.0 &     1.46 &  $-$0.88 &  \ldots &    91.1 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 5662.16 & 22.0 &     2.32 &  $-$0.05 &    67.0 &    78.8 &  \ldots &  \ldots &    84.5 &  \ldots &  \ldots &    51.0 &  \ldots \\
 5866.45 & 22.0 &     1.07 &  $-$0.78 &   113.9 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    99.2 &  \ldots \\
 5880.27 & 22.0 &     1.05 &  $-$1.99 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    26.8 &  \ldots &  \ldots \\
 5899.30 & 22.0 &     1.05 &  $-$1.10 &   104.4 &  \ldots &  \ldots &   117.0 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 5903.33 & 22.0 &     1.05 &  $-$2.09 &    38.0 &    65.6 &    62.8 &    52.9 &    72.4 &   124.9 &    25.6 &    26.0 &   115.2 \\
 5922.11 & 22.0 &     1.05 &  $-$1.41 &    81.7 &   109.5 &    90.5 &    95.0 &   116.2 &  \ldots &    56.7 &  \ldots &  \ldots \\
 5965.83 & 22.0 &     1.88 &  $-$0.35 &  \ldots &   105.8 &    88.3 &    94.7 &  \ldots &  \ldots &    57.9 &    66.6 &  \ldots \\
 5978.54 & 22.0 &     1.87 &  $-$0.44 &    75.2 &    92.8 &    80.1 &    83.2 &    97.0 &  \ldots &    51.5 &    56.1 &  \ldots \\
 6064.63 & 22.0 &     1.05 &  $-$1.89 &    55.4 &    80.2 &    62.5 &    68.6 &    88.3 &  \ldots &    33.6 &    33.7 &  \ldots \\
 6091.17 & 22.0 &     2.27 &  $-$0.37 &    55.1 &    74.3 &    60.6 &  \ldots &    77.1 &   122.6 &  \ldots &  \ldots &   114.4 \\
 6092.80 & 22.0 &     1.89 &  $-$1.32 &    25.4 &  \ldots &    31.0 &    37.6 &  \ldots &   105.5 &  \ldots &  \ldots &  \ldots \\
 6126.22 & 22.0 &     1.07 &  $-$1.37 &    88.5 &  \ldots &    94.9 &   102.4 &   117.5 &  \ldots &    62.4 &    65.1 &  \ldots \\
 6258.10 & 22.0 &     1.44 &  $-$0.30 &   105.4 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 6261.10 & 22.0 &     1.43 &  $-$0.42 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    92.0 &  \ldots &  \ldots \\
 6303.76 & 22.0 &     1.44 &  $-$1.51 &    50.5 &    70.7 &  \ldots &    62.4 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 6312.24 & 22.0 &     1.46 &  $-$1.50 &    46.8 &    72.2 &    62.4 &    62.1 &    76.5 &  \ldots &  \ldots &  \ldots &  \ldots \\
 6336.10 & 22.0 &     1.44 &  $-$1.69 &    35.9 &    59.4 &    51.1 &    50.2 &    71.8 &  \ldots &    29.8 &    22.7 &  \ldots \\
 6554.22 & 22.0 &     1.46 &  $-$1.02 &    76.8 &    83.6 &    91.5 &    85.8 &   102.7 &  \ldots &    53.1 &  \ldots &  \ldots \\
 6556.06 & 22.0 &     1.44 &  $-$1.07 &    78.6 &  \ldots &  \ldots &    94.0 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 6599.13 & 22.0 &     0.90 &  $-$2.03 &    61.0 &    87.9 &    70.5 &    75.3 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 4545.14 & 22.1 &     1.13 &  $-$1.81 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   100.5 &  \ldots &  \ldots \\
 4568.31 & 22.1 &     1.22 &  $-$2.52 &    66.0 &    80.0 &    73.1 &    77.8 &    75.8 &   101.5 &  \ldots &    69.9 &  \ldots \\
 4583.44 & 22.1 &     1.17 &  $-$2.77 &  \ldots &    75.9 &    69.5 &  \ldots &  \ldots &  \ldots &  \ldots &    68.6 &    76.5 \\
 4589.96 & 22.1 &     1.24 &  $-$1.75 &  \ldots &   118.2 &  \ldots &   117.5 &  \ldots &  \ldots &   107.1 &   120.7 &  \ldots \\
 4609.26 & 22.1 &     1.18 &  $-$3.26 &  \ldots &    66.2 &    69.8 &    64.6 &    69.5 &  \ldots &    44.5 &    56.1 &  \ldots \\
 4708.66 & 22.1 &     1.24 &  $-$2.30 &    75.8 &  \ldots &  \ldots &    88.5 &  \ldots &   108.2 &  \ldots &  \ldots &  \ldots \\
 4779.99 & 22.1 &     2.05 &  $-$1.38 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    91.7 &  \ldots \\
 4794.81 & 22.1 &     1.13 &  $-$4.05 &     6.9 &  \ldots &  \ldots &     9.4 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 4865.62 & 22.1 &     1.12 &  $-$2.74 &    72.0 &    89.2 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    81.8 &  \ldots \\
 4874.03 & 22.1 &     3.10 &  $-$0.99 &    50.1 &    52.7 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 4981.36 & 22.1 &     1.57 &  $-$3.16 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    40.7 &  \ldots \\
 5005.16 & 22.1 &     1.57 &  $-$2.54 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    81.1 &  \ldots &  \ldots &    67.7 \\
 5185.90 & 22.1 &     1.89 &  $-$1.56 &  \ldots &  \ldots &  \ldots &    99.1 &  \ldots &  \ldots &  \ldots &    98.6 &  \ldots \\
 5336.81 & 22.1 &     1.58 &  $-$1.70 &    98.1 &   102.6 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   105.3 &  \ldots \\
 5492.86 & 22.1 &     1.58 &  $-$3.31 &    35.8 &    40.8 &  \ldots &    40.6 &  \ldots &  \ldots &    27.6 &    31.7 &  \ldots \\
 5910.05 & 22.1 &     1.57 &  $-$3.24 &    73.6 &  \ldots &  \ldots &  \ldots &    88.9 &  \ldots &  \ldots &  \ldots &  \ldots \\
 6214.60 & 22.1 &     2.05 &  $-$2.03 &  \ldots &  \ldots &  \ldots &  \ldots &    40.4 &  \ldots &  \ldots &  \ldots &  \ldots \\
 6606.95 & 22.1 &     2.06 &  $-$2.83 &    27.0 &  \ldots &    34.5 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 6013.53 & 25.0 &     3.07 &  $-$0.25 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   100.9 &   108.7 &  \ldots \\
 6016.67 & 25.0 &     3.08 &  $-$0.10 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   107.1 &   118.2 &  \ldots \\
 6021.80 & 25.0 &     3.08 &     0.03 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   108.9 &   118.6 &  \ldots \\
 4439.88 & 26.0 &     2.28 &  $-$3.00 &  \ldots &    97.7 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 4602.00 & 26.0 &     1.61 &  $-$3.15 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    98.9 &   104.2 &  \ldots \\
 4802.88 & 26.0 &     3.69 &  $-$1.53 &    81.2 &  \ldots &    87.6 &    81.4 &    84.5 &   116.1 &    71.8 &    79.4 &    83.4 \\
 4962.57 & 26.0 &     4.18 &  $-$1.20 &  \ldots &  \ldots &  \ldots &    75.1 &  \ldots &  \ldots &  \ldots &    68.5 &  \ldots \\
 5044.21 & 26.0 &     2.85 &  $-$2.03 &  \ldots &  \ldots &  \ldots &   114.7 &  \ldots &  \ldots &    90.8 &    98.0 &  \ldots \\
 5054.64 & 26.0 &     3.64 &  $-$1.94 &  \ldots &    73.8 &  \ldots &    61.8 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 5141.74 & 26.0 &     2.42 &  $-$2.00 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   106.0 &   116.5 &  \ldots \\
 5217.39 & 26.0 &     3.21 &  $-$1.18 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   114.6 &  \ldots &  \ldots \\
 5223.19 & 26.0 &     3.63 &  $-$1.80 &  \ldots &  \ldots &    69.7 &  \ldots &  \ldots &   113.2 &  \ldots &  \ldots &  \ldots \\
 5242.49 & 26.0 &     3.63 &  $-$0.98 &   108.3 &   115.0 &   117.7 &   113.0 &   118.0 &  \ldots &    93.0 &   106.5 &   123.2 \\
 5253.46 & 26.0 &     3.28 &  $-$1.63 &   100.6 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    98.0 &  \ldots \\
 5267.28 & 26.0 &     4.37 &  $-$1.66 &  \ldots &    55.5 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 5288.53 & 26.0 &     3.69 &  $-$1.53 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    71.1 &  \ldots &  \ldots \\
 5307.36 & 26.0 &     1.61 &  $-$2.99 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   119.3 &  \ldots &  \ldots \\
 5321.11 & 26.0 &     4.43 &  $-$1.11 &    54.0 &  \ldots &    66.2 &    62.6 &    61.4 &    95.0 &    47.4 &  \ldots &    83.4 \\
 5322.04 & 26.0 &     2.28 &  $-$2.84 &   100.1 &   110.6 &   113.1 &   115.4 &   114.9 &  \ldots &    86.5 &    95.2 &  \ldots \\
 5326.14 & 26.0 &     3.57 &  $-$2.13 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    60.2 &    94.3 \\
 5365.40 & 26.0 &     3.57 &  $-$1.04 &  \ldots &   106.9 &  \ldots &   111.3 &  \ldots &  \ldots &  \ldots &  \ldots &   123.9 \\
 5367.48 & 26.0 &     4.41 &     0.43 &  \ldots &  \ldots &  \ldots &    95.2 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 5379.57 & 26.0 &     3.69 &  $-$1.53 &  \ldots &    95.8 &  \ldots &  \ldots &  \ldots &   106.4 &  \ldots &  \ldots &   107.7 \\
 5491.84 & 26.0 &     4.18 &  $-$2.25 &    22.4 &    28.3 &  \ldots &    25.9 &    28.6 &    56.5 &    16.0 &    17.2 &    43.0 \\
 5525.54 & 26.0 &     4.23 &  $-$1.15 &    72.4 &    79.3 &    82.6 &  \ldots &    77.6 &    74.5 &    66.1 &  \ldots &  \ldots \\
 5618.63 & 26.0 &     4.21 &  $-$1.29 &    67.0 &    68.7 &    71.8 &  \ldots &    69.6 &  \ldots &  \ldots &    65.6 &  \ldots \\
 5661.35 & 26.0 &     4.28 &  $-$1.82 &    39.1 &    46.6 &    55.1 &    45.0 &    50.1 &  \ldots &    30.4 &    32.2 &  \ldots \\
 5701.55 & 26.0 &     2.56 &  $-$2.22 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   108.3 &   119.3 &  \ldots \\
 5705.47 & 26.0 &     4.30 &  $-$1.42 &    57.0 &    61.7 &  \ldots &  \ldots &    69.2 &    70.0 &    50.0 &  \ldots &  \ldots \\
 5741.85 & 26.0 &     4.25 &  $-$1.69 &    48.7 &    55.9 &    58.4 &    49.7 &    53.1 &    56.4 &    38.6 &    45.0 &    72.2 \\
 5775.08 & 26.0 &     4.22 &  $-$1.31 &    77.3 &    84.9 &    86.8 &    79.6 &    84.1 &    88.8 &    66.9 &    71.7 &    91.5 \\
 5778.45 & 26.0 &     2.59 &  $-$3.48 &  \ldots &    76.2 &    71.4 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 5811.92 & 26.0 &     4.14 &  $-$2.43 &    23.3 &    27.3 &    29.3 &    28.8 &    28.2 &  \ldots &    19.3 &    18.8 &    37.6 \\
 5837.70 & 26.0 &     4.29 &  $-$2.34 &    20.8 &    20.9 &    28.1 &    21.8 &    22.5 &  \ldots &    15.1 &    13.5 &  \ldots \\
 5853.16 & 26.0 &     1.49 &  $-$5.28 &    42.7 &    58.0 &    51.4 &    53.3 &    65.8 &   104.7 &    30.4 &    28.9 &    90.8 \\
 5855.09 & 26.0 &     4.60 &  $-$1.55 &    29.0 &    33.9 &    38.3 &    38.0 &    40.9 &    60.2 &    25.4 &    28.4 &    48.1 \\
 5856.10 & 26.0 &     4.29 &  $-$1.64 &    49.6 &    57.9 &    58.6 &  \ldots &  \ldots &  \ldots &    40.0 &  \ldots &  \ldots \\
 5858.79 & 26.0 &     4.22 &  $-$2.26 &  \ldots &    31.3 &    31.8 &    31.0 &  \ldots &  \ldots &    19.6 &    19.5 &    46.2 \\
 5909.97 & 26.0 &     3.21 &  $-$2.64 &    73.6 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    60.4 &    64.4 &  \ldots \\
 5916.25 & 26.0 &     2.45 &  $-$2.99 &    97.3 &  \ldots &   108.2 &  \ldots &  \ldots &  \ldots &    82.5 &    89.1 &  \ldots \\
 5927.80 & 26.0 &     4.65 &  $-$1.09 &    52.6 &    62.4 &    63.6 &    64.3 &    60.0 &    74.1 &    46.2 &    54.3 &    72.0 \\
 5933.80 & 26.0 &     4.64 &  $-$2.23 &     9.1 &  \ldots &    18.9 &  \ldots &    20.3 &  \ldots &  \ldots &  \ldots &  \ldots \\
 5956.69 & 26.0 &     0.86 &  $-$4.61 &   119.2 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    95.4 &   101.7 &  \ldots \\
 5969.58 & 26.0 &     4.28 &  $-$2.73 &    10.8 &  \ldots &  \ldots &  \ldots &    15.2 &    23.4 &  \ldots &  \ldots &    19.6 \\
 6012.21 & 26.0 &     2.22 &  $-$4.07 &    64.5 &    75.6 &    73.7 &  \ldots &    75.5 &  \ldots &    47.4 &    49.0 &   103.1 \\
 6019.36 & 26.0 &     3.57 &  $-$3.36 &    13.1 &    22.6 &    26.5 &    29.0 &    28.3 &    40.0 &    15.1 &  \ldots &    37.4 \\
 6027.05 & 26.0 &     4.07 &  $-$1.11 &    90.1 &  \ldots &  \ldots &  \ldots &    92.9 &  \ldots &    79.0 &  \ldots &    99.1 \\
 6054.08 & 26.0 &     4.37 &  $-$2.31 &    21.4 &    19.7 &    22.8 &  \ldots &    28.6 &  \ldots &    14.8 &  \ldots &    34.5 \\
 6105.13 & 26.0 &     4.55 &  $-$2.05 &  \ldots &    23.6 &    29.8 &    29.3 &  \ldots &    33.0 &  \ldots &  \ldots &    36.8 \\
 6120.24 & 26.0 &     0.91 &  $-$5.97 &    43.6 &    61.2 &    52.2 &    54.6 &    65.3 &   115.5 &    26.5 &    25.9 &    99.1 \\
 6145.42 & 26.0 &     3.37 &  $-$3.60 &  \ldots &    13.3 &    13.3 &  \ldots &    15.6 &  \ldots &  \ldots &     6.1 &    26.3 \\
 6151.62 & 26.0 &     2.17 &  $-$3.30 &    93.9 &   107.9 &   106.0 &   109.6 &   113.4 &  \ldots &    78.8 &    82.3 &  \ldots \\
 6159.38 & 26.0 &     4.61 &  $-$1.97 &    23.3 &    30.7 &    30.9 &    31.0 &  \ldots &  \ldots &    22.4 &    19.9 &    45.8 \\
 6165.36 & 26.0 &     4.14 &  $-$1.49 &    69.3 &    72.9 &    74.5 &  \ldots &    71.7 &  \ldots &    53.1 &    57.4 &    85.3 \\
 6173.34 & 26.0 &     2.22 &  $-$2.88 &   115.5 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    95.2 &   105.6 &  \ldots \\
 6200.31 & 26.0 &     2.61 &  $-$2.44 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   100.2 &   108.0 &  \ldots \\
 6229.23 & 26.0 &     2.84 &  $-$2.85 &    84.8 &    85.9 &    83.2 &  \ldots &    91.3 &  \ldots &    63.9 &    66.8 &   102.7 \\
 6232.64 & 26.0 &     3.65 &  $-$1.28 &   107.0 &   119.0 &  \ldots &   122.9 &  \ldots &  \ldots &    95.4 &  \ldots &  \ldots \\
 6246.32 & 26.0 &     3.60 &  $-$0.89 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   116.8 &  \ldots &  \ldots \\
 6270.22 & 26.0 &     2.86 &  $-$2.50 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    77.2 &    78.8 &  \ldots \\
 6271.28 & 26.0 &     3.33 &  $-$2.76 &  \ldots &    60.6 &  \ldots &  \ldots &    62.0 &  \ldots &    41.7 &    39.0 &  \ldots \\
 6297.79 & 26.0 &     2.22 &  $-$2.74 &   111.6 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   100.9 &   115.7 &  \ldots \\
 6301.50 & 26.0 &     3.65 &  $-$0.77 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   113.6 &  \ldots &  \ldots \\
 6322.69 & 26.0 &     2.59 &  $-$2.43 &   117.3 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   100.2 &   111.1 &  \ldots \\
 6336.82 & 26.0 &     3.68 &  $-$0.92 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   110.1 &   117.1 &  \ldots \\
 6353.84 & 26.0 &     0.91 &  $-$6.48 &  \ldots &    37.0 &  \ldots &  \ldots &    36.6 &  \ldots &  \ldots &  \ldots &  \ldots \\
 6469.19 & 26.0 &     4.84 &  $-$0.77 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    67.4 &    73.2 &  \ldots \\
 6481.87 & 26.0 &     2.28 &  $-$2.98 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   103.9 &  \ldots \\
 6498.94 & 26.0 &     0.96 &  $-$4.69 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    94.3 &    99.2 &  \ldots \\
 6518.36 & 26.0 &     2.83 &  $-$2.50 &    93.6 &   107.7 &   100.8 &  \ldots &   107.3 &  \ldots &  \ldots &  \ldots &  \ldots \\
 6574.23 & 26.0 &     0.99 &  $-$5.00 &    94.7 &   114.4 &   100.3 &   113.7 &  \ldots &  \ldots &    73.3 &    79.1 &  \ldots \\
 6575.02 & 26.0 &     2.59 &  $-$2.73 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    91.1 &  \ldots \\
 6593.87 & 26.0 &     2.43 &  $-$2.42 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   119.1 &  \ldots &  \ldots \\
 6648.08 & 26.0 &     1.01 &  $-$5.92 &    54.2 &    76.4 &    64.6 &  \ldots &    76.0 &   116.6 &  \ldots &  \ldots &   115.4 \\
 6699.16 & 26.0 &     4.59 &  $-$2.17 &  \ldots &    28.7 &    20.8 &  \ldots &    20.2 &    34.7 &    13.4 &  \ldots &    28.5 \\
 6739.52 & 26.0 &     1.56 &  $-$4.82 &    57.0 &    72.9 &    64.7 &    67.2 &    75.9 &  \ldots &    37.0 &    41.2 &   113.6 \\
 6750.15 & 26.0 &     2.42 &  $-$2.62 &   116.9 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   102.5 &   108.5 &  \ldots \\
 6756.56 & 26.0 &     4.29 &  $-$2.75 &  \ldots &  \ldots &    11.1 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 6810.26 & 26.0 &     4.60 &  $-$1.00 &    66.3 &    68.5 &    70.7 &    73.8 &    73.7 &  \ldots &    56.4 &    62.6 &    80.2 \\
 6837.02 & 26.0 &     4.59 &  $-$1.76 &    32.4 &  \ldots &    34.9 &    32.8 &    39.1 &    44.4 &  \ldots &  \ldots &  \ldots \\
 6971.93 & 26.0 &     3.02 &  $-$3.39 &  \ldots &  \ldots &  \ldots &    50.5 &  \ldots &    74.3 &  \ldots &  \ldots &    77.6 \\
 7112.17 & 26.0 &     2.99 &  $-$3.04 &  \ldots &    84.8 &    86.3 &  \ldots &    81.4 &  \ldots &    56.7 &    62.0 &   109.5 \\
 7189.15 & 26.0 &     3.07 &  $-$2.80 &  \ldots &  \ldots &    77.1 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 7223.66 & 26.0 &     3.01 &  $-$2.27 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    87.7 &    94.4 &  \ldots \\
 7401.69 & 26.0 &     4.18 &  $-$1.66 &  \ldots &    66.7 &    53.7 &  \ldots &  \ldots &    74.9 &  \ldots &  \ldots &    79.5 \\
 7710.36 & 26.0 &     4.22 &  $-$1.13 &    85.4 &    92.9 &    87.3 &  \ldots &    90.6 &    91.6 &    72.6 &    81.9 &  \ldots \\
 7723.20 & 26.0 &     2.28 &  $-$3.62 &    83.4 &   105.4 &    85.3 &  \ldots &   105.3 &  \ldots &    72.1 &    77.0 &  \ldots \\
 7941.09 & 26.0 &     3.27 &  $-$2.33 &    75.5 &    85.7 &    86.1 &    88.7 &    89.4 &   107.5 &    64.8 &    67.0 &   108.3 \\
 8075.15 & 26.0 &     0.91 &  $-$5.09 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    97.9 &  \ldots \\
 4491.40 & 26.1 &     2.85 &  $-$2.68 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    88.5 &  \ldots &  \ldots \\
 4508.29 & 26.1 &     2.85 &  $-$2.31 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &   100.1 &  \ldots \\
 4576.34 & 26.1 &     2.84 &  $-$2.82 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    84.5 &  \ldots \\
 4620.52 & 26.1 &     2.83 &  $-$3.08 &    63.0 &  \ldots &    69.0 &    64.7 &  \ldots &  \ldots &    61.8 &    70.0 &  \ldots \\
 4993.36 & 26.1 &     2.81 &  $-$3.49 &    50.1 &    57.0 &    53.3 &    52.5 &    54.5 &  \ldots &    48.2 &    57.7 &    61.3 \\
 5234.62 & 26.1 &     3.22 &  $-$2.15 &    86.4 &    80.5 &  \ldots &    95.2 &  \ldots &  \ldots &    86.3 &   102.1 &  \ldots \\
 5325.55 & 26.1 &     3.22 &  $-$3.22 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    56.4 &    48.1 \\
 5991.38 & 26.1 &     3.15 &  $-$3.56 &    47.6 &  \ldots &    50.0 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    47.0 \\
 6084.11 & 26.1 &     3.20 &  $-$3.81 &  \ldots &  \ldots &    31.7 &    33.8 &    31.1 &    29.5 &    29.4 &    33.5 &    33.9 \\
 6149.26 & 26.1 &     3.89 &  $-$2.72 &    35.2 &    33.3 &    40.6 &    41.8 &    34.8 &  \ldots &    38.6 &    42.5 &  \ldots \\
 6247.56 & 26.1 &     3.89 &  $-$2.33 &    45.3 &    41.9 &    56.0 &  \ldots &    43.1 &  \ldots &    50.7 &    57.3 &  \ldots \\
 6369.46 & 26.1 &     2.89 &  $-$4.25 &    27.8 &    30.4 &    31.9 &    31.1 &    22.9 &    40.2 &  \ldots &    31.9 &    34.1 \\
 6383.72 & 26.1 &     5.55 &  $-$2.27 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    10.5 &  \ldots &  \ldots \\
 6416.92 & 26.1 &     3.89 &  $-$2.74 &    45.7 &    43.5 &    50.7 &  \ldots &    35.6 &  \ldots &    39.1 &    48.9 &  \ldots \\
 6432.68 & 26.1 &     2.89 &  $-$3.71 &    47.7 &    49.9 &    57.3 &  \ldots &    45.4 &    58.4 &    49.8 &    57.2 &    48.7 \\
 6456.38 & 26.1 &     3.90 &  $-$2.08 &  \ldots &    62.7 &    75.3 &  \ldots &    55.4 &    42.9 &    66.3 &    70.7 &    51.0 \\
 6516.08 & 26.1 &     2.89 &  $-$3.45 &  \ldots &  \ldots &    69.8 &  \ldots &    60.3 &  \ldots &    64.3 &    68.5 &  \ldots \\
 7224.49 & 26.1 &     3.89 &  $-$3.24 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    11.6 &    32.9 &    33.2 &  \ldots \\
 7711.72 & 26.1 &     3.90 &  $-$2.54 &    37.8 &  \ldots &    47.6 &  \ldots &    41.3 &  \ldots &    47.4 &    52.7 &    43.4 \\
 6189.00 & 27.0 &     1.71 &  $-$2.45 &  \ldots &    93.1 &    74.6 &    82.4 &    96.7 &  \ldots &    44.7 &    47.2 &  \ldots \\
 6455.03 & 27.0 &     3.63 &  $-$0.25 &  \ldots &    49.1 &    43.5 &    44.5 &    51.5 &  \ldots &    30.8 &    31.0 &    73.3 \\
 6632.45 & 27.0 &     2.28 &  $-$2.00 &    45.6 &    55.4 &    47.1 &    44.8 &    60.4 &    84.8 &    28.4 &    28.0 &    85.5 \\
 5846.99 & 28.0 &     1.68 &  $-$3.21 &    68.3 &    85.7 &    87.8 &    77.8 &    91.7 &   123.6 &    55.8 &    59.1 &  \ldots \\
 6086.28 & 28.0 &     4.26 &  $-$0.52 &    51.5 &    58.3 &    56.2 &    62.5 &    57.9 &    52.8 &    47.6 &    51.8 &    67.2 \\
 6175.37 & 28.0 &     4.09 &  $-$0.54 &    60.3 &    63.8 &    67.1 &    61.7 &    68.1 &  \ldots &    53.4 &    57.9 &    70.2 \\
 6177.24 & 28.0 &     1.83 &  $-$3.51 &    55.9 &  \ldots &    59.9 &    61.6 &  \ldots &  \ldots &    39.0 &    38.9 &    88.2 \\
 6204.60 & 28.0 &     4.09 &  $-$1.14 &  \ldots &    41.0 &    46.9 &  \ldots &    44.6 &  \ldots &    28.9 &    28.1 &  \ldots \\
 6635.12 & 28.0 &     4.42 &  $-$0.83 &    41.8 &    36.0 &    42.0 &    44.2 &    40.4 &  \ldots &    33.3 &    33.7 &  \ldots \\
 6772.32 & 28.0 &     3.66 &  $-$0.99 &    59.0 &    70.7 &    80.1 &    72.6 &    73.9 &   114.6 &    64.3 &    65.4 &  \ldots \\
 6127.44 & 40.0 &     0.15 &  $-$1.06 &    30.5 &    50.8 &    38.2 &    44.6 &  \ldots &  \ldots &    13.9 &    16.6 &   112.7 \\
 6134.55 & 40.0 &     0.00 &  $-$1.28 &    22.6 &    46.3 &    37.6 &    34.3 &    49.6 &  \ldots &    10.1 &    10.1 &   115.5 \\
 6143.20 & 40.0 &     0.07 &  $-$1.10 &    23.9 &    47.4 &    37.2 &    40.3 &    53.7 &  \ldots &    12.0 &    11.7 &   122.3 \\
 5853.64 & 56.1 &     0.60 &  $-$1.01 &   109.9 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    99.2 &  \ldots &  \ldots \\
 5805.77 & 57.1 &     0.13 &  $-$1.56 &    37.1 &    47.0 &    50.1 &    50.0 &    50.9 &    67.0 &    35.6 &    33.6 &    71.6 \\
 6390.48 & 57.1 &     0.32 &  $-$1.41 &    27.0 &    37.0 &    39.7 &    46.0 &    39.0 &   109.6 &    18.8 &    19.0 &    74.8 \\
 6645.11 & 63.1 &     1.38 &     0.20 &    28.3 &    34.3 &    30.6 &    34.1 &    37.8 &    52.6 &    21.4 &    25.1 &    53.5 \\
\enddata

\end{deluxetable}



==> tab13.tex <==
\begin{deluxetable}{llrrrrrrrrrrrrrrrrrrr}
\centering
\tabletypesize{\tiny}
\setlength{\voffset}{1.0in}
\tablecolumns{9} 
\tablewidth{0pc} 
\tablecaption{Compilation of (LTE) Abundance Ratios for Open Clusters \label{tab:compile}}
\tablehead{ 
\colhead{} & 
\colhead{} &
\colhead{Age\tablenotemark{a}} &
\colhead{Distance\tablenotemark{a}} &
\colhead{Age\tablenotemark{b}} &
\colhead{Distance\tablenotemark{b}} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} \\

\colhead{Cluster} & 
\colhead{Source} &
\colhead{(Gyr)} &
\colhead{(kpc)} &
\colhead{(Gyr)} &
\colhead{(kpc)} &
\colhead{[Fe/H]} &
\colhead{[O/Fe]} &
\colhead{[Na/Fe]} &
\colhead{[Mg/Fe]} &
\colhead{[Al/Fe]} &
\colhead{[Si/Fe]} &
\colhead{[Ca/Fe]} &
\colhead{[Ti/Fe]} &
\colhead{[Mn/Fe]} &
\colhead{[Co/Fe]} &
\colhead{[Ni/Fe]} &
\colhead{[Zr/Fe]} &
\colhead{[Ba/Fe]} &
\colhead{[La/Fe]} &
\colhead{[Eu/Fe]} 
}
\startdata
Be 17 & Friel10 & 10.10 & 11.70 & 10.06 & 10.89 & $-$0.10 & 0.00 & 0.33 & 0.12 & 0.25 & 0.30 & $-$0.04 & 0.02 & \ldots & \ldots & 0.02 & \ldots & \ldots & \ldots & \ldots \\
Be 18 & This Study & 5.69 & 13.10 & 5.69 & 12.09 & $-$0.44 & 0.11 & 0.21 & 0.18 & 0.19 & 0.17 & 0.12 & 0.19 & $-$0.10 & 0.19 & $-$0.02 & $-$0.21 & 0.30 & 0.34 & 0.30 \\
Be 20 & Sestito08 & 6.00 & 16.37 & 4.05 & 16.12 & $-$0.30 & \ldots & 0.17 & 0.28 & 0.17 & 0.05 & 0.07 & 0.13 & \ldots & \ldots & 0.03 & \ldots & 0.16 & \ldots & \ldots \\
Be 20 & Y05 & 4.10 & 16.00 & 4.05 & 16.12 & $-$0.49 & 0.18 & 0.21 & 0.24 & 0.18 & 0.06 & 0.07 & 0.39 & $-$0.12 & 0.18 & $-$0.02 & 0.05 & 0.14 & 0.30 & 0.31 \\
Be 21 & This Study & 2.18 & 14.27 & 2.18 & 14.27 & $-$0.31 & 0.18 & 0.36 & 0.19 & 0.17 & 0.21 & 0.20 & 0.20 & 0.11 & 0.15 & 0.07 & $-$0.11 & 0.58 & 0.56 & 0.31 \\
Be 21 & Hill99 & 2.18 & 14.27 & 2.18 & 14.27 & $-$0.53 & \ldots & 0.45 & \ldots & 0.20 & 0.32 & $-$0.10 & 0.29 & \ldots & \ldots & $-$0.03 & \ldots & \ldots & \ldots & \ldots \\
Be 22 & This Study & 4.26 & 11.92 & 4.26 & 11.92 & $-$0.45 & 0.17 & 0.42 & 0.18 & 0.39 & 0.19 & 0.25 & 0.35 & $-$0.22 & 0.19 & 0.10 & $-$0.14 & 0.60 & 0.38 & 0.26 \\
Be 22 & Villanova05 & \ldots & \ldots & 4.26 & 11.92 & $-$0.32 & \ldots & 0.03 & \ldots & 0.29 & 0.04 & $-$0.08 & 0.12 & \ldots & \ldots & 0.05 & \ldots & \ldots & \ldots & \ldots \\
Be 25 & Carraro07 & 5.00 & 18.20 & \ldots & \ldots & $-$0.20 & \ldots & \ldots & 0.11 & \ldots & $-$0.01 & $-$0.19 & 0.04 & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
Be 29 & Carraro04 & 4.50 & 21.60 & 4.34 & 18.72 & $-$0.44 & 0.18 & 0.39 & $-$0.01 & 0.21 & 0.22 & 0.11 & 0.03 & \ldots & \ldots & 0.11 & \ldots & \ldots & \ldots & \ldots \\
Be 29 & Y05 & 4.30 & 22.50 & 4.34 & 18.72 & $-$0.54 & 0.23 & 0.37 & 0.34 & 0.26 & 0.18 & 0.02 & 0.33 & $-$0.23 & 0.09 & $-$0.02 & 0.07 & 0.31 & 0.23 & 0.16 \\
Be 29 & Sestito08 & 4.00 & 22.00 & 4.34 & 18.72 & $-$0.31 & \ldots & 0.11 & 0.18 & 0.05 & 0.03 & 0.10 & 0.08 & \ldots & \ldots & $-$0.03 & \ldots & 0.43 & \ldots & \ldots \\
Be 31 & Y05 & 5.30 & 12.90 & 5.32 & 12.02 & $-$0.53 & 0.24 & 0.27 & 0.40 & 0.22 & 0.20 & 0.13 & 0.08 & $-$0.54 & 0.25 & 0.11 & 0.35 & 0.64 & 0.91 & 0.56 \\
Be 32 & Bragaglia08 & 5.91 & 11.30 & 5.91 & 11.30 & $-$0.29 & \ldots & 0.14 & 0.27 & 0.11 & 0.12 & 0.07 & 0.09 & \ldots & \ldots & 0.00 & \ldots & 0.29 & \ldots & \ldots \\
Be 32 & Friel10 & 5.90 & 11.60 & 5.91 & 11.30 & $-$0.30 & $-$0.01 & 0.20 & 0.13 & 0.19 & 0.27 & $-$0.07 & $-$0.17 & \ldots & 0.00 & $-$0.02 & $-$0.23 & \ldots & \ldots & \ldots \\
Be 32 & This Study & 5.91 & 11.30 & 5.91 & 11.30 & $-$0.38 & 0.23 & 0.24 & 0.21 & 0.18 & 0.20 & 0.15 & 0.26 & $-$0.05 & 0.15 & 0.04 & $-$0.06 & 0.28 & 0.44 & 0.31 \\
Be 39 & Friel10 & 7.00 & 11.90 & 7.00 & 11.71 & $-$0.21 & $-$0.02 & 0.11 & 0.15 & 0.20 & 0.19 & $-$0.01 & $-$0.03 & \ldots & $-$0.09 & $-$0.04 & 0.02 & \ldots & \ldots & \ldots \\
Be 66 & Villanova05 & \ldots & \ldots & 3.98 & 12.59 & $-$0.48 & \ldots & 0.15 & \ldots & 0.01 & \ldots & $-$0.05 & 0.43 & \ldots & \ldots & 0.24 & \ldots & \ldots & \ldots & \ldots \\
Be 73 & Carraro07 & 1.50 & 17.40 & \ldots & \ldots & $-$0.22 & \ldots & \ldots & 0.10 & \ldots & 0.17 & $-$0.08 & 0.05 & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
Be 75 & Carraro07 & 4.00 & 15.50 & \ldots & \ldots & $-$0.22 & \ldots & \ldots & 0.38 & \ldots & $-$0.20 & $-$0.02 & 0.16 & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
Cr 110 & Pancino10 & 1.70\tablenotemark{c} & 9.74\tablenotemark{c} & \ldots & \ldots & 0.03 & 0.03 & $-$0.06 & 0.16 & $-$0.04 & 0.04 & $-$0.07 & 0.02 & \ldots & 0.01 & $-$0.02 & \ldots & 0.49 & 0.03 & \ldots \\
Cr 261 & Carretta05 & 6.00 & 7.52 & 8.00 & 7.49 & $-$0.03 & $-$0.12 & 0.33 & 0.17 & 0.12 & 0.24 & 0.01 & $-$0.09 & $-$0.03 & 0.01 & 0.06 & \ldots & 0.30 & \ldots & \ldots \\
Cr 261 & de Silva07 & \ldots & \ldots & 8.00 & 7.49 & $-$0.01 & \ldots & 0.13 & 0.14 & \ldots & 0.19 & 0.01 & \ldots & $-$0.03 & \ldots & $-$0.03 & $-$0.03 & 0.02 & \ldots & 0.01 \\
Cr 261 & Sestito08 & 6.00 & 7.52 & 8.00 & 7.49 & 0.13 & \ldots & 0.06 & 0.20 & 0.26 & 0.09 & $-$0.04 & 0.10 & \ldots & \ldots & 0.07 & \ldots & 0.28 & \ldots & \ldots \\
Hyades & Paulson03, & \ldots & \ldots & 0.70 & 8.55 & 0.13 & \ldots & $-$0.12 & $-$0.19 & \ldots & $-$0.08 & $-$0.06 & \ldots & $-$0.13 & \ldots & $-$0.13 & $-$0.06 & 0.37 & \ldots & $-$0.13 \\
 & de Silva06 & &  &  &  &  &  &  &  &  &  &  &  & &  &  &  & & &  \\
IC 4651 & Carretta04 & 1.68 & 7.65 & 1.68 & 7.65 & 0.11 & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
M67 & Friel10 & 4.30 & 9.10 & 4.30 & 9.05 & 0.03 & $-$0.16 & 0.14 & 0.05 & 0.11 & 0.18 & $-$0.08 & $-$0.14 & \ldots & $-$0.16 & $-$0.02 & $-$0.14 & \ldots & \ldots & \ldots \\
M67 & Jacobson11b & 4.30 & 9.09  & 4.30 & 9.05 & $-$0.01 & $-$0.11 & 0.03 & 0.23 & 0.36 & 0.21 & $-$0.11 & $-$0.10 & \ldots & \ldots & $-$0.01 & $-$0.03 & \ldots & \ldots & \ldots \\
M67 & Y05 & 4.30 & 8.60 & 4.30 & 9.05 & 0.02 & 0.07 & 0.30 & 0.16 & 0.17 & 0.09 & 0.07 & 0.12 & $-$0.13 & 0.02 & 0.08 & $-$0.28 & $-$0.02 & 0.11 & 0.06 \\
Mel 66 & Sestito08 & 4.00 & 10.21 & 5.33 & 9.44 & $-$0.33 & \ldots & 0.19 & 0.31 & 0.29 & 0.13 & 0.11 & 0.02 & \ldots & \ldots & $-$0.01 & \ldots & 0.33 & \ldots & \ldots \\
NGC 188 & Friel10 & 6.30 & 9.40 & 6.30 & 9.35 & 0.12 & $-$0.04 & 0.15 & 0.15 & 0.20 & 0.17 & $-$0.03 & 0.05 & \ldots & 0.09 & $-$0.03 & 0.15 & \ldots & \ldots & \ldots \\
NGC 188 & Jacobson11b & 6.30 & 9.40 & 6.30 & 9.35 & $-$0.03 & \ldots & 0.10 & 0.26 & \ldots & 0.25 & $-$0.04 & 0.14 & \ldots & \ldots & 0.08 & 0.00 & \ldots & \ldots & \ldots \\
NGC 752 & Carrera11 & 0.65 & \ldots & 1.24 & 8.75 & 0.08 & 0.03 & 0.01 & 0.12 & $-$0.12 & 0.02 & $-$0.09 & $-$0.03 & \ldots & 0.01 & $-$0.01 & \ldots & 0.52 & 0.18 & \ldots \\
NGC 1193 & Friel10 & 4.20 & 13.60 & 4.23 & 12.00 & $-$0.22 & $-$0.08 & 0.25 & 0.23 & 0.10 & 0.16 & 0.11 & 0.10 & \ldots & $-$0.15 & 0.01 & 0.20 & \ldots & \ldots & \ldots \\
NGC 1245 & Jacobson11b & 1.10 & 11.10 & 1.06 & 11.09 & $-$0.04 & 0.08 & 0.04 & 0.09 & \ldots & 0.18 & 0.05 & $-$0.09 & \ldots & \ldots & $-$0.02 & 0.33 & \ldots & \ldots & \ldots \\
NGC 1817 & Friel10 & 1.10 & 10.00 & 1.12 & 10.26 & $-$0.07 & $-$0.19 & 0.12 & 0.01 & 0.01 & 0.12 & 0.06 & $-$0.06 & \ldots & $-$0.26 & $-$0.11 & 0.21 & \ldots & \ldots & \ldots \\
NGC 1817 & Jacobson11b & 1.10 & 10.00 & 1.12 & 10.26 & $-$0.16 & $-$0.02 & 0.11 & 0.08 & \ldots & 0.17 & 0.07 & $-$0.06 & \ldots & \ldots & $-$0.05 & 0.34 & \ldots & \ldots & \ldots \\
NGC 1883 & Friel10 & 0.70 & 12.30 & \ldots & \ldots & $-$0.01 & $-$0.22 & 0.04 & $-$0.04 & $-$0.12 & 0.15 & $-$0.05 & $-$0.10 & \ldots & $-$0.27 & $-$0.13 & $-$0.11 & \ldots & \ldots & \ldots \\
NGC 2099 & Pancino10 & 0.43\tablenotemark{c} & 9.26\tablenotemark{c} & \ldots & \ldots & 0.01 & 0.15 & 0.09 & 0.27 & $-$0.06 & 0.09 & $-$0.08 & $-$0.08 & \ldots & $-$0.04 & $-$0.02 & \ldots & 0.57 & 0.09 & \ldots \\
NGC 2141 & Y05 & 2.50 & 11.80 & 2.45 & 12.60 & $-$0.14 & 0.00 & 0.41 & 0.24 & 0.18 & 0.05 & 0.10 & 0.24 & $-$0.20 & 0.04 & 0.04 & 0.63 & 0.91 & 0.57 & 0.17 \\
NGC 2141 & Friel10 & 2.40 & 12.20 & 2.45 & 12.60 & 0.00 & $-$0.15 & 0.15 & 0.03 & 0.01 & 0.14 & $-$0.11 & $-$0.05 & \ldots & $-$0.26 & $-$0.11 & $-$0.13 & \ldots & \ldots & \ldots \\
NGC 2158 & Friel10 & 1.90 & 12.80 & 1.91 & 12.36 & $-$0.03 & $-$0.17 & 0.10 & $-$0.02 & $-$0.03 & 0.12 & $-$0.06 & $-$0.05 & \ldots & $-$0.29 & $-$0.04 & $-$0.05 & \ldots & \ldots & \ldots \\
NGC 2158 & Jacobson11b & 1.90 & 12.50 & 1.91 & 12.36 & $-$0.28 & 0.03 & 0.01 & 0.22 & 0.38 & 0.39 & 0.00 & $-$0.26 & \ldots & \ldots & 0.05 & 0.00 & \ldots & \ldots & \ldots \\
NGC 2194 & Jacobson11b & 0.90 & 10.30 & 0.87 & 11.06 & $-$0.08 & \ldots & 0.04 & 0.00 & \ldots & 0.18 & $-$0.03 & $-$0.24 & \ldots & \ldots & $-$0.03 & 0.22 & \ldots & \ldots & \ldots \\
NGC 2204 & Jacobson11a & 2.00 & 11.60 & \ldots & \ldots & $-$0.23 & \ldots & \ldots & \ldots & 0.12 & 0.16 & \ldots & $-$0.40 & \ldots & \ldots & 0.01 & \ldots & \ldots & \ldots & \ldots \\
NGC 2243 & Jacobson11a & 4.70 & 10.70 & 4.66 & 10.76 & $-$0.42 & \ldots & 0.03 & 0.18 & 0.21 & 0.24 & 0.13 & $-$0.10 & \ldots & \ldots & 0.01 & 0.06 & \ldots & \ldots & \ldots \\
NGC 2324 & Bragaglia08 & 0.67 & 11.29 & 0.67 & 11.29 & $-$0.17 & \ldots & 0.36 & 0.25 & 0.00 & 0.06 & 0.15 & 0.00 & \ldots & \ldots & $-$0.09 & \ldots & 0.62 & \ldots & \ldots \\
NGC 2355 & Jacobson11b & 0.80 & 10.30 & 0.79 & 10.52 & $-$0.08 & \ldots & 0.05 & 0.21 & \ldots & 0.19 & 0.05 & $-$0.04 & \ldots & \ldots & 0.02 & 0.24 & \ldots & \ldots & \ldots \\
NGC 2420 & Jacobson11b & 2.20 & 10.70 & 2.20 & 10.59 & $-$0.20 & $-$0.01 & 0.08 & 0.11 & \ldots & 0.21 & 0.10 & $-$0.07 & \ldots & \ldots & $-$0.01 & 0.24 & \ldots & \ldots & \ldots \\
NGC 2420 & Pancino10 & \ldots & \ldots & 2.20 & 10.59 & $-$0.05 & 0.15 & $-$0.04 & 0.09 & $-$0.10 & 0.04 & $-$0.09 & $-$0.04 & \ldots & 0.03 & 0.00 & \ldots & 0.62 & 0.23 & \ldots \\
NGC 2425 & Jacobson11b & 2.50 & 10.60 & \ldots & \ldots & $-$0.15 & \ldots & 0.14 & 0.07 & \ldots & 0.20 & 0.17 & 0.06 & \ldots & \ldots & 0.00 & 0.33 & \ldots & \ldots & \ldots \\
NGC 2477 & Bragaglia08 & 1.00 & 8.89 & 1.00 & 8.89 & 0.07 & \ldots & 0.17 & 0.07 & $-$0.01 & 0.05 & $-$0.01 & 0.04 & \ldots & \ldots & 0.00 & \ldots & 0.46 & \ldots & \ldots \\
NGC 2506 & Carretta04 & 2.14 & 10.81 & 2.14 & 10.81 & $-$0.20 & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
NGC 2660 & Bragaglia08 & 0.73 & 9.18 & 0.73 & 9.18 & 0.04 & \ldots & 0.13 & 0.15 & $-$0.08 & 0.00 & 0.04 & 0.03 & \ldots & \ldots & $-$0.03 & \ldots & 0.61 & \ldots & \ldots \\
NGC 3960 & Bragaglia08 & 0.90 & 7.96 & \ldots & \ldots & 0.02 & \ldots & 0.16 & 0.13 & $-$0.06 & 0.04 & 0.02 & 0.01 & \ldots & \ldots & $-$0.01 & \ldots & 0.54 & \ldots & \ldots \\
NGC 6253 & Carretta07 & 3.00 & 6.60 & \ldots & \ldots & 0.46 & $-$0.18 & 0.21 & 0.01 & $-$0.08 & 0.09 & $-$0.02 & \ldots & 0.04 & \ldots & $-$0.05 & \ldots & 0.16 & \ldots & 0.03 \\
NGC 6253 & Sestito08 & 3.00 & 6.60 & \ldots & \ldots & 0.36 & \ldots & 0.20 & 0.28 & \ldots & $-$0.01 & 0.01 & 0.02 & \ldots & \ldots & 0.05 & \ldots & 0.23 & \ldots & \ldots \\
NGC 6791 & Carretta07 & 10.20 & 8.18 & 10.20 & 8.12 & 0.47 & $-$0.31 & 0.13 & 0.20 & $-$0.21 & $-$0.01 & $-$0.15 & 0.03 & 0.08 & \ldots & $-$0.07 & \ldots & 0.28 & \ldots & $-$0.17 \\
NGC 6819 & Bragaglia01 & 2.91 & 8.18 & 2.91 & 8.18 & 0.09 & \ldots & 0.47 & $-$0.12 & $-$0.07 & \ldots & $-$0.04 & $-$0.01 & \ldots & $-$0.08 & \ldots & \ldots & $-$0.27 & \ldots & \ldots \\
NGC 7142 & Friel10 & 4.00 & 9.20 & 4.04 & 9.70 & 0.14 & $-$0.10 & 0.24 & 0.07 & 0.14 & 0.09 & $-$0.02 & 0.04 & \ldots & $-$0.03 & $-$0.02 & 0.22 & \ldots & \ldots & \ldots \\
NGC 7789 & Jacobson11b & 1.80 & 9.60 & 1.80 & 9.44 & 0.02 & 0.08 & 0.09 & 0.14 & \ldots & 0.25 & 0.01 & $-$0.05 & \ldots & \ldots & 0 & 0.18 & \ldots & \ldots & \ldots \\
NGC 7789 & Pancino10 & \ldots & \ldots & 1.80 & 9.44 & 0.04 & 0.16 & $-$0.05 & 0.22 & $-$0.03 & $-$0.01 & $-$0.18 & $-$0.03 & \ldots & $-$0.02 & $-$0.01 & \ldots & 0.45 & 0.11 & \ldots \\
NGC 7789 & Tautvai{\v s}ien{\.e}05 & \ldots & \ldots & 1.80 & 9.44 & $-$0.04 & $-$0.07 & 0.28 & 0.18 & 0.18 & 0.14 & 0.14 & $-$0.03 & \ldots & 0.09 & $-$0.02 & \ldots & \ldots & \ldots & \ldots \\
Praesepe & Carrera11 & 1.59 & \ldots & 0.70 & 8.62 & 0.16 & $-$0.11 & 0.25 & 0.27 & 0.00 & 0.06 & $-$0.08 & $-$0.07 & \ldots & 0.04 & 0.02 & \ldots & 0.33 & $-$0.05 & \ldots \\
PWM4 & This Study & 7.00 & 13.50 & \ldots & \ldots & $-$0.34 & 0.18 & 0.42 & 0.23 & 0.26 & 0.10 & 0.19 & 0.14 & $-$0.28 & 0.13 & $-$0.03 & 0.11 & 0.46 & 0.22 & 0.12 \\
Ruprecht~4 & Carraro07 & 0.80 & 12.40 & \ldots & \ldots & $-$0.09 & \ldots & \ldots & 0.01 & \ldots & 0.05 & 0.05 & 0.04 & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
Ruprecht~7 & Carraro07 & 0.80 & 13.50 & \ldots & \ldots & $-$0.26 & \ldots & \ldots & $-$0.10 & \ldots & 0.05 & 0.03 & $-$0.12 & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
Saurer 1 & Carraro04 & 5.00 & 19.20 & \ldots & \ldots & $-$0.38 & 0.42 & 0.44 & 0.03 & 0.33 & 0.38 & 0.20 & 0.13 & \ldots & \ldots & 0.20 & \ldots & \ldots & \ldots & \ldots \\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\\
\enddata

\tablenotetext{a}{Ages and distances taken from the individual papers}
\tablenotetext{b}{Ages and distances taken from \citet{salaris04}}
\tablenotetext{c}{Ages and distances taken from \citet{bragaglia06}}

\tablerefs{
Bragaglia01 = \citet{bragaglia01}; 
Bragaglia08 = \citet{bragaglia08};
Carraro04 = \citet{carraro04}; 
Carrera11 = \citet{carrera11}; \\
Carretta04 = \citet{carretta04};
Carretta05 = \citet{carretta05};
Carretta07 = \citet{carretta07};
de Silva06 = \citet{desilva06}; \\
de Silva07 = \citet{desilva07}; 
Friel10 = \citet{friel05,jacobson08,jacobson09,friel10}; 
Hill99 = \citet{hill99}; 
Jacobson11a = \citet{jacobson11a};\\
Jocobson11b = \citet{jacobson11b}; 
Pancino10 = \citet{pancino10}; 
Paulson03 = \citet{paulson03};
Sestito08 = \citet{sestito06,sestito07,sestito08,bragaglia08}; 
Villanova05 = \citet{villanova05}; 
Y05 = \citet{y05}}
\end{deluxetable}


